Real and complex dynamics of a family of birational maps of the plane: the golden mean subshift

We give a detailed description of the dynamics of a family of birational mappings of the plane. The organizing theme of our analysis is that this family is essentially conjugate to the golden mean subshift.

==> texfiles/oldintro.tex <==
\noindent  
There are several recent examples of problems in math and physics 
that reduce to questions about iterating specific families of multivariable 
rational maps.  This seems to happen frequently, for instance,
with problems concerning integrable systems and discrete analogues for
differential equations (see \cite{Saka, BeVi, RaGr} and some
of the references therein).  And in these cases, the maps that occur
usually come with additional structure, such as an invariant meromorphic two 
form, that does not exist for typical rational maps.  The dynamics
of typical rational maps of $\C^n$, on the other hand, has been a subject of 
interest in its own right, and both the results and the techniques used
to achieve them have seen significant progress in the past decade.  Our goal 
in this paper is to show by example how techniques used to study general 
rational maps might be specialized to shed light on some of the specific 
families that arise in applications.

\mpar{Some unresolved points:  

I still have to add some references (Friday,
I hope).  Please
suggest any that seem good---especially for the introduction.  

I prefer `Fibonacci' subshift to `golden mean' or `golden ratio'
subshift.  What about you?  If we go with Fibonacci, should I change
$\Sigma_G$ to something like $\Sigma_F$ throughout?

I haven't yet changed $R(w)'$ to $R'(w)$.  Do you still prefer this?

There are a couple of marginal notes for you in the body of the paper.
}

Our immediate object of interest is the one parameter family of birational maps
$$
f_a(x,y)=(y\frac{x+a}{x-1}, x+a-1),
$$
which has its origin in physical models from thermodynamics and 
has received a great deal of numerical scrutiny in a series of 
physics papers (see \cite{Abetal} and its references).  For negative values of 
the parameter $a$,
we will describe the real dynamics of $f_a$ in a very
concrete and precise fashion.  Though $f_a$ is not continuously defined 
everywhere nor hyperbolic in the dynamical systems sense, the picture that
emerges is quite similar to that of a smooth hyperbolic system.  On its 
nonwandering set $f_a$ turns out to be essentially conjugate to the `Fibonacci 
subshift.'

It is most convenient for us to regard $f = f_a$ as a birational self-map of
the compact complex surface $\pp$.  The point $(\infty,\infty)$ is fixed and
parabolic for $f$ regardless of the parameter $a$, and it plays a
very important role in the dynamics.  We assume as indicated above that
$a$ is real and negative.  Then $f$ restricts to a dynamical system 
$f:\overline{\R^2}\self$ acting on the real points in $\pp$.
Moreover, there are closed rectangles $R_+, R_-\subset\overline{\R^2}$ that
determine whether and in what manner an orbit converges to $(\infty,\infty)$ 
in forward or backward time.  

\begin{thm}[see Proposition \ref{thm1} and Theorem \ref{thm2}]
$f(R_+)\subset R_+$ and $\lim_{n\to\infty} f^n(p) = (\infty,\infty)$ if and 
only if $f^n(p)\in R_+$ for some $n\geq 0$.  Likewise, 
$f^{-1}(R_-)\subset R_-$ and $\lim_{n\to\infty} f^{-n}(p) = (\infty,\infty)$ 
if and only if $f^{-n}(p)\in R_+$ for some $n\geq 0$
\end{thm}

\noindent
The reader should note our imprecision here.
Because $f$ is merely birational, there are points like $(0,1)$ where
$f$ is indeterminate and cannot be defined as a continuous map.  For now we 
will disregard the difficulties 
concerning such points.  In subsequent sections, we will be more careful.

The complement of $R_+\cup R_-$ consists of disjoint open rectangles,
The closures $R_0$ and $R_1$ of these rectangles intersect only at 
$(\infty,\infty)$.  In light of the theorem above, 
we see that the most interesting orbits for $f$ are those
entirely contained in $R_0\cup R_1$.  Let $\Omega$ denote the (obviously
invariant) union of such orbits.  When $a=-1$, the map $f$ is linear
and $\Omega = \{(\infty,\infty)\}$, so we discard this case.  Otherwise any 
point $p\in\Omega-(\infty,\infty)$ can be `coded' 
with a `word' $\dots w_{-2}w_{-1}w_0\cdot w_1w_2\dots$, whose digits
$w_k\in\{0,1\}$ are chosen by the condition $f^k(p)\in R_{w_k}$.  The action
of $f$ on $\Omega$ corresponds to left shift 
$$
\sigma(\dots w_{-2}w_{-1}w_0\cdot w_1w_2\dots) = 
       \dots w_{-2}w_{-1}w_0w_1\cdot w_2\dots 
$$
on the word.  

An easy computation concerning the images of $R_0$ and $R_1$ 
reveals (Proposition \ref{thm1}) that codings never contain
consecutive 1's.  More careful scrutiny (Proposition \ref{allowables})
shows that this necessary condition is also sufficient (Corollary 
\ref{nonempty}), i.e. any word $w = \dots w_{-1}w_0.w_1\dots$ with no 
consecutive 1's codes some orbit in $\Omega$.
We call such words \emph{admissable} and let $\Sigma_G$ denote
the set of all admissable words endowed with the product topology.  
The shift map $\sigma:\Sigma_G\self$ is a homeomorphism that we
refer to as the \emph{Fibonacci subshift}.
The results described so far imply that coding
orbits in $\Omega$ with words in $\Sigma_G$ (essentially) 
semiconjugates $f:\Omega\self$ to $\sigma:\Sigma_G\self$.  
The proofs require little or no reference to the larger complex setting.

However, we take tremendous advantage of the complex setting 
when we show that the semiconjugacy is
(essentially) a conjugacy.  The proof that every word in $\Sigma_G$ codes
an orbit in $\Omega$ relies on a lower bound for the number of
intersections between certain well-chosen curves.  These (real)
curves can be chosen as the real slices of complex varieties in $\pp$.  
Complex intersection theory exactly counts the complex intersections of the 
varieties, and therefore provides an upper bound for the number of  
intersections between the real slices.  The upper and lower bounds turn
out to agree, so in the end we are able to account very precisely for
each intersection we are interested in.  We use this device repeatedly
and in various ways throughout Sections \ref{productstructure}, 
\ref{boundary}, and \ref{periodic}.  Along the way we show

\begin{thm}[see Theorems \ref{saddles}]
$\Omega$ contains all periodic points of $f$.  In particular, all
periodic points are real.  Finally, all periodic points except 
$(\infty,\infty)$ are saddles.
\end{thm}

After further analysis of the behavior of orbits that pass near 
$(\infty,\infty)$ in Section \ref{parabolic}, we arrive at the key
result that the coding map is injective 
on $\Omega\cap\R^2$.  In Section \ref{conjugacy}, we state most of the 
central results of the paper.  Some of these are summarized in
the next few paragraphs.

\begin{thm}[see Theorem \ref{nonwandering}] $\Omega$ is the non-wandering 
set of
$f|_{\overline{\R^2}}$.
\end{thm}

The set $\Omega$ includes points of indeterminacy for iterates of
$f$, and as we noted earlier, these complicate things considerably.  
However, none of these bad points are finite and all of them are
attracted to $(\infty,\infty)$ in forward or backward time.  In order to 
proceed, we introduce some notation.
Let $\Omega'$ denote $\Omega\cap\R^2$ and $\Omega''$ denote 
$\Omega'$ with the critical set $\cC(f^n)$ of $f^n$ removed for every 
$n\in\Z$.  The point $(\infty,\infty)$ corresponds by way of coding to the 
unique two cycle 
$$
\overline{10}.\overline{10} \leftrightarrow \overline{01}.\overline{01}
$$
in $\Sigma_G$.  Let $\Sigma_G'\subset\Sigma_G$ denote the complement 
of the local stable and unstable sets of this two cycle.  Finally, let 
$\Sigma_G''\subset\Sigma_G'$ be obtained by further excluding the global
stable and unstable sets.

\begin{thm}[See Corollary \ref{finiteomega} and Theorem \ref{conjdomain}] 
There is a natural homeomorphism 
$$
\Omega' \to \Sigma_G'
$$
conjugating $f:\Omega''\self$ to $\sigma:\Sigma_G''\self$.
\end{thm}

The dynamics of the Fibonacci subshift are well-understood, so
this theorem implies a great deal of about the dynamics of $f$.

\begin{thm}[see Theorem \ref{entropy}]
The topological entropy of $f:\pp\self$ is $\log\frac{1+\sqrt{5}}{2}$.  
This coincides
with the topological entropy of $f$ restricted to $\overline{\R^2}$ or
to $\Omega$.
\end{thm}

The variational principle says that topological entropy of $f$ is the
least upper bound of the entropies associated to $f$-invariant measures.
In our case the least upper bound is realized.

\begin{thm}[see Corollary \ref{mu} and Theorem \ref{unique}]
Let $\Per(n)$ denote the periodic points of period $n$ for $f$.  
Then the limit
$$
\mu = \lim_{n\to\infty} \frac{1}{\#\Per(n)}\sum_{p\in\Per(n)} \delta_p
$$ 
exists and defines an ergodic $f$-invariant with 
$\supp\mu = \overline{\Omega'}$.  Moreover,
$\mu$ is the unique invariant measure supported on $\overline{\R^2}$
with (maximal) entropy $\log\frac{1+\sqrt{5}}{2}$.  
\end{thm}

In Section \ref{currents} we describe the stable set $\Omega^+$ of
$\Omega$.  The finite part $\Omega^+\cap\R^2$ turns out (see
Theorem \ref{lamination}) to be homeomorphic to 
the product of an interval with a Cantor set.  Because of this we
are able to define a laminar 1-current $\mu^+_{\R}$ with 
$\supp\mu^+_{\R} = \Omega^+$ 
that transforms according to the formula 
$f^*\mu^+_{\R} = \pm\lambda\mu^+_{\R}$, according to whether $a$ is less
or greater than $-1$, respectively.
Using $\mu^+_{\R}$ and the analogous current $\mu^-_{\R}$ supported on the 
unstable
set of $\Omega$, we recover the measure $\mu_{\R}$ as a `geometric
intersection' $\mu^+_{\R}\wedge\mu^-_{\R}$.

While the results of this paper hold for all $a<0$ except $a=-1$, we
only give full proofs for the case $a<-1$.  The proofs are similar for
the case $-1<a<0$, but in Section \ref{smallnega} we point out those
few places in which the case $-1<a<0$ differs enough to warrant mention.

In Section \ref{complex}, we compare the results of this paper with
more general results concerning complex dynamics of birational maps.
It is probably impossible to describe the dynamics of a typical birational 
map
in anything like the level of detail we are able to provide for the
family of maps considered here.  However, the real currents $\mu^+_{\R}$ and 
$\mu^-_{\R}$ have perfectly general complex analogues, and in most cases
one can again construct an invariant measure $\mu$ by making sense of the
product $\mu^+\wedge\mu^-$.  In the family we consider here, both the
real and complex constructions yield the same measure 
(Theorem \ref{samemeasure}).

By way of context, let us recall another place where complex
analytic tools have been used to treat real dynamics---namely, the
H\'enon family of diffeomorphisms of ${\bf R}^2$:
$$h_{a,b}(x,y)=(y,y^2+a-bx).$$
It is known (see Devaney-Nitecki \cite{DeNi} and Hubbard-ObersteVorth 
\cite{HuOb}) that
$h_{a,b}$ is conjugate to a horseshoe map for a large open subset
of parameters $(a,b)$.  The horesehoes are examples of real quadratic 
maps whose entropy is equal to $\log 2$, which is the maximum possible 
for a quadratic diffeomorphism.  Indeed the dynamics of a horseshoe on its 
nonwandering set is conjugate to the dynamics of the \emph{full} shift
on two symbols.

The maps $f_a$, $a<0$, $a\ne-1$ that we consider in this paper have maximal 
complexity
within the family $\{f_a\}_{a\in\C}$.  They therefore occupy a position
analogous to that of the horseshoes in the H\'enon family.  Unlike 
horseshoes, however,
the entropy $\log\lambda$ of $f_a$ is not the logarithm of an integer,
and the dynamics of
$f_a$ cannot be those of a full shift on finitely many symbols.  
Moreover, the nonwandering set of $f_a$ always includes
the parabolic point $(\infty,\infty)$, and thus $f_a$ is not hyperbolic.  




